SafeShift: Safety-Informed Distribution Shifts for Robust Trajectory Prediction in Autonomous Driving

As autonomous driving technology matures, safety and robustness of its key components, including trajectory prediction, is vital. Though real-world datasets, such as Waymo Open Motion, provide realistic recorded scenarios for model development, they often lack truly safety-critical situations. Rather than utilizing unrealistic simulation or dangerous real-world testing, we instead propose a framework to characterize such datasets and find hidden safety-relevant scenarios within. Our approach expands the spectrum of safety-relevance, allowing us to study trajectory prediction models under a safety-informed, distribution shift setting. We contribute a generalized scenario characterization method, a novel scoring scheme to find subtly-avoided risky scenarios, and an evaluation of trajectory prediction models in this setting. We further contribute a remediation strategy, achieving a 10% average reduction in prediction collision rates. To facilitate future research, we release our code to the public: github.com/cmubig/SafeShift

==> sections/4_bak.tex <==
% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.5\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/individual_corrmat.png}
%          \caption{$y=x$}
%          \label{fig:y equals x}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.5\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{figures/interaction_corrmat.png}
%          \caption{$y=3\sin x$}
%          \label{fig:three sin x}
%      \end{subfigure}
%      \hfill
%     \caption{Three simple graphs}
%     \label{fig:three graphs}
% \end{figure}



\section{Scenario Features} \label{sec:approach}
%\rev{3}{3}{\bs{We should have either an algorithm outlining our feature extraction and scoring or also a diagram showing how the components are built up. Can do a better version of Figure 5 in \cite{glasmacher2022automated}. We should also more thoroughly enumerate the score variants, of GT only, FE, Asym, etc.} It is difficult to understand the contributions 1 and 2 from Section 4. There is very limited detail about the implementation. It is strongly suggested to revise Section 3 and 4 with more equations, figures and algorithm tables.}

%\rev{1}{4}{\bs{Same as above; make it more accessible via clearer text, algorithm descriptions, and diagrams. Could also have a figure demonstrating what certain metrics look like} The approach, particularly the scoring strategy, may be considered complex for readers without a strong background in autonomous driving or machine learning.}
%\bs{Add in figures + bullet points + equations to make it easier to understand}


We propose a hierarchical scheme as in~\cite{glasmacher2022automated, sadat2021diverse}, where low-level, base features are computed within a scenario and then later aggregated to form an overall score to represent a scenario's overall safety-relevance.

%\bs{make this point clearer, that we're using the scoring/characterization for two key things: creating distribution shift, i.e., a harder evaluation setting; and improving prediction performance/safety/robustness in this new setting}

\subsection{Dataset Preprocessing}\label{sec:preprocessing}

We consider base features across two main categories: individual and social. For both of these categories, accurate lane assignment is highly important.
%Understanding which lane an agent is traveling along is non-trivial, particularly when lanes are represented as polylines. Furthermore, certain agent types, such as pedestrians or cyclists, may not adhere to lanes.
Understanding which lane an agent is traveling along is non-trivial, especially as VRUs often do not adhere to lanes. Thus, we leverage a probabilistic approach based on \cite{schmidt2022meat} to find valid lane \textit{sequences}. We permit lane assignments based on physically plausible lane deflection angles rather than the lane connectivity graph alone. %For robustness against lane graph errors, as well as to allow for situations such as crossing the median to avoid an obstacle, we permit lane assignments based on physically plausible lane deflection angles.

%Additionally, we note that not all self-driving datasets provide the same information. For instance, Argoverse~\cite{chang2019argoverse} provides global, city coordinates, which models can directly leverage, whereas WOMD~\cite{ettinger2021large} only provides scene-local coordinates. As such,

Note that many features utilized in previous frameworks and datasets~\cite{glasmacher2022automated, moers2022exid}, such as driving region-based anomaly detection, cannot be used as they rely on global, city coordinates unavailable in all AD datasets. Instead, to identify anomalies, we utilize a traffic primitive extraction and clustering approach pioneered in \cite{guha2022robust}. This process produces cluster centers for both single trajectories and trajectory pairs, allowing us to easily measure anomalies.

%\bs{Potentially expand on this? Was low key non-trivial} 


%\task{Especially for subsections A and B, does it read as novel enough compared to the other frameworks, especially ``An automated analysis framework for trajectory datasets''~\cite{glasmacher2022automated}}

\subsection{Feature Extraction and Analysis}

%\bs{Shorten this and refer people to figure 2 for the full list. Maybe briefly mention which papers these come from?}

For individual features, we primarily focus on metrics derived from relative positional data of a trajectory, such as speed, acceleration, and jerk. We additionally implement metrics to incorporate map context, including waiting period (WP)~\cite{zhan2019interaction}, speed difference with the lane's speed limit, and the percentage of time that the agent is following a lane. Finally, we include a trajectory anomaly value, derived from its distance to the nearest   \textit{individual} traffic primitive cluster. %from \Cref{sec:preprocessing}.

For social features, we use widely studied and accepted safety surrogate metrics, as in \cite{glasmacher2022automated, vogel2003comparison, shen2020crash}. These include time headway (THW), time-to-collision (TTC), deceleration rate to avoid crash (DRAC), and the difference between minimum time to conflict points ($\Delta$mTTCP) %. 
%As noted in \cite{vogel2003comparison}, THW mostly represents a stable car-following scenario, whereas TTC characterizes more critical scenarios. Additionally, TTC and DRAC have been used for assessing rear-end crash risk~\cite{shen2020crash}.
%These metrics are then complemented by $\Delta$mTTCP, to incorporate future conflict points 
in both agent trajectories as well as roadgraph locations of interest (\exempli crosswalks, stop signs, etc.). 
We then incorporate a measure of collisions directly, counting situations where two agents' center points or segmented paths overlap at a given timestep. Finally, we add in a trajectory-pair anomaly value analogously to \textit{individual}, using the paired traffic primitive clusters.% from \Cref{sec:preprocessing}.
%\bs{Potentially add more information about these metrics, maybe even some equations?}

%\task{Provide a table to list these metrics, instead of in paragraph form?}

\begin{figure}[t!]
    \vspace{0.2cm}
    \centering
    \includegraphics[width=0.49\textwidth,trim={0cm 0cm -0cm -0cm},clip]{figures/scores_0.png}
    \vspace{-0.2cm}
    \caption{PDF of our score variations, exhibiting long-tailed behavior. Analysis performed in WOMD~\cite{ettinger2021large}.}
    \vspace{-0.2cm}
    \label{fig:score_dist}
\end{figure}

\input{tables/score_variations}


%\subsection{Feature Analysis}

%As discussed in \Cref{sec:problem_definition}, we utilize WOMD~\cite{ettinger2021large} as a representative dataset to justify our feature selection.
Our full feature selection, along with a correlation analysis, is shown in \Cref{fig:correlation_analysis}. For the individual features, the kinematic-based ones correlate positively, as could be expected, while the other features are largely weakly correlated. Similarly, for the social features, TTC and THW have a weak correlation, as they both involve a leader-follower scenario. The two forms of $\Delta$mTTCP are also relatively strongly correlated, as agent trajectories are required to be somewhat intertwined for both. This analysis implies that the selection and extraction of base features are largely complementary, without excessive overlap in coverage. %\task{Refine discussion of implications from this.}

\begin{figure*}[t]
    \vspace{0.2cm}
    \centering
    \includegraphics[width=\textwidth,trim={0cm 0cm -0cm -0cm},clip]{figures/scene_scores_v4.png}
    \caption{Examples of scenes by score. In-Distribution and Out-of-Distribution follow our \texttt{Scoring} split in \Cref{sec:dataset_implementation}.}
    \vspace{-0.5cm}
    \label{fig:scored_scenes}
\end{figure*}

%\subsection{Feature Aggregation}


==> tables/main_table_v1.tex <==

\begin{table*}[!ht]
\centering
\caption{\ina{In progress; improving / simplifying table layout.} Main Experiments} \label{tab:results_main}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{c@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}}
\begin{tabular}{clcccccccc}
\toprule
\multirow{2}{*}{\textbf{Data Split}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c}{\textbf{Remediation Strategy}} & \multicolumn{3}{c}{\textbf{Val Set}} & \multicolumn{3}{c}{\textbf{Test Set}}  \\ 
\cmidrule(l){3-4} \cmidrule(l){5-7} \cmidrule(l){8-10}
 & & F+ & X & ADE / FDE ($\downarrow$) & mAP ($\uparrow$) & Collisions ($\downarrow$) & ADE / FDE ($\downarrow$) & mAP ($\uparrow$) & Collisions ($\downarrow$) \\ 
\midrule
\multirow{3}{*}{Uniform} & MTR & & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
                         & MotionCNN & & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
                         & A-VRNN & & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
\midrule[0.7pt]
\multirow{9}{*}{Fr\'enet Clusters} & \multirow{3}{*}{MTR} & & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
                                 & & $\checkmark$ & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
                                 & & & $\checkmark$ & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\ \cmidrule(l){2-10}
                                 & \multirow{3}{*}{MotionCNN} & & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
                                 & & $\checkmark$ & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
                                 & & & $\checkmark$ & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\ \cmidrule(l){2-10}
                                 & \multirow{3}{*}{A-VRNN} & & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
                                 & & $\checkmark$ & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
                                 & & & $\checkmark$ & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
\midrule[0.7pt]
\multirow{9}{*}{Scoring (Ours)} & \multirow{3}{*}{MTR} & & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
                                 & & $\checkmark$ & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
                                 & & & $\checkmark$ & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\ \cmidrule(l){2-10}
                                 & \multirow{3}{*}{MotionCNN} & & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
                                 & & $\checkmark$ & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
                                 & & & $\checkmark$ & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\ \cmidrule(l){2-10}
                                 & \multirow{3}{*}{A-VRNN} & & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
                                 & & $\checkmark$ & & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
                                 & & & $\checkmark$ & X / X & X & X & X (X\%) / X (+X\%) & X (X\%) & X (X\%) \\
\bottomrule
\end{tabular}
}
\begin{tablenotes}
\scriptsize
\item \textbf{F+}: Fren\'et+ Strategy, \textbf{SC}: Scoring strategy (Ours)
\end{tablenotes}
% \vspace{-0.2cm}
\end{table*}

==> tables/main_table_v2.tex <==

\begin{table*}[!ht]
\centering
\caption{Main Experiments: values for ADE / FDE are in meters, collisions are rates per predicted trajectory} \label{tab:results_main}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{c@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}}
\begin{tabular}{clccccccc}
\toprule
\multirow{2}{*}{\textbf{Data Split}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Remediation}} & \multicolumn{3}{c}{\textbf{Validation Set (In-Distribution)}} & \multicolumn{3}{c}{\textbf{Testing Set (Out-of-Distribution)}}  \\ 
%\cmidrule(l){4-6} \cmidrule(l){7-9}
 & & & ADE / FDE ($\downarrow$) & mAP ($\uparrow$) & Collisions ($\downarrow$) & ADE / FDE ($\downarrow$) & mAP ($\uparrow$) & Collisions ($\downarrow$) \\ 
\midrule
\multirow{4}{*}{\texttt{Uniform}} 
     & GT & - & 0.00 / 0.00 & 1.00 & 0.008 & 0.00 / 0.00 & 1.00 & 0.009 \\
     \cmidrule(l){2-9}
     & MTR~\cite{shi2022motion}  & - & 0.73 / 1.58 & 0.30 & 0.062 & 0.73 / 1.59 & 0.31 & 0.061 \\
     & MotionCNN~\cite{konev2022motioncnn} & - & 0.70 / 1.48 & 0.13 & 0.055 & 0.71 / 1.49  & 0.13  & 0.056  \\
     & A-VRNN~\cite{monti2020dagnet}  & - & 1.80 / 4.63 & 0.06 & 0.057 & 1.82 / 4.67  & 0.06  & 0.058  \\
\midrule[0.7pt]

\multirow{4}{*}{\texttt{Clusters}~\cite{ye2023improving}} 
     & GT & - & 0.00 / 0.00 & 1.00 & 0.009 & 0.00 / 0.00 & 1.00 & 0.007 \\
     \cmidrule(l){2-9}
     & MTR~\cite{shi2022motion} & - & 0.69 / 1.50 & 0.35 & 0.060 & 0.71 / 1.55 & 0.33 & 0.051 \\
     & MotionCNN~\cite{konev2022motioncnn}  & - & 0.77 / 1.63 & 0.13 & 0.056 & 0.78 / 1.65  & 0.12  & 0.047  \\
     & A-VRNN~\cite{monti2020dagnet}  & - & 1.79 / 4.59 & 0.08 & 0.062 & 1.82 / 4.70  & 0.07  & 0.049 \\
\midrule[0.7pt]

\multirow{10}{*}{\texttt{Scoring}} 
     & GT & - & 0.00 / 0.00 & 1.00 & 0.005 & 0.00 / 0.00 & 1.00 & 0.017 \\
 \cmidrule(l){2-9}
& \multirow{3}{*}
    {MTR~\cite{shi2022motion}}  & - &    0.72 / 1.59 & 0.32 & 0.044 & 0.74 / 1.59  & 0.30  & 0.100  \\
     & & F+~\cite{ye2023improving} &       0.73 / 1.59 & 0.32 & 0.043 & 0.75 / 1.59  & 0.30  & 0.099  \\
     &  & Ours &   0.83 / 1.80 & 0.25 & 0.037 & 0.89 / 1.91  & 0.22  & 0.086  \\ 
     \cmidrule(l){2-9}
& \multirow{3}{*}
    {MotionCNN~\cite{konev2022motioncnn}}  & - &    0.71 / 1.51 & 0.14 & 0.037 & 0.73 / 1.55  & 0.13 & 0.089  \\
     & & F+~\cite{ye2023improving} &             0.76 / 1.64 & 0.14 & 0.038 & 0.78 / 1.67  & 0.13  & 0.089  \\
     &  & Ours &          0.75 / 1.60 & 0.20 & 0.038 & 0.77 / 1.64  & 0.18  & 0.091  \\ 
     \cmidrule(l){2-9}
& \multirow{3}{*}
    {A-VRNN~\cite{monti2020dagnet}}  & - &    1.99 / 5.26 & 0.05 & 0.042 & 2.13 / 5.55  & 0.05 & 0.099  \\
     & & F+~\cite{ye2023improving} &             2.05 / 5.24 & 0.06 & 0.041 & 2.23 / 5.73  & 0.06  & 0.103  \\
     &  & Ours &          1.76 / 4.58 & 0.07 & 0.041 & 1.89 / 4.87 & 0.06 & 0.095  \\ 
\bottomrule
\end{tabular}
}
\begin{tablenotes}
\scriptsize
\item \textbf{GT}: Ground truth tracks, \textbf{F+}: Fren\'et+ Strategy~\cite{ye2023improving}
\end{tablenotes}
% \vspace{-0.2cm}
\end{table*}

==> tables/main_table_v3.tex <==

\begin{table*}[!ht]
\centering
\caption{Main Experiments in WOMD~\cite{ettinger2021large}: values for ADE / FDE are in meters, collisions are rates per predicted trajectory} \label{tab:results_main}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{c@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}}
\begin{tabular}{clccccccc}
\toprule
\multirow{2}{*}{\textbf{Data Split}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Remediation}} & \multicolumn{3}{c}{\textbf{Validation Set (In-Distribution)}} & \multicolumn{3}{c}{\textbf{Testing Set (Out-of-Distribution)}}  \\ 
%\cmidrule(l){4-6} \cmidrule(l){7-9}
 & & & ADE / FDE ($\downarrow$) & mAP ($\uparrow$) & Collisions ($\downarrow$) & ADE / FDE ($\downarrow$) & mAP ($\uparrow$) & Collisions ($\downarrow$) \\ 
\midrule
\multirow{4}{*}{\texttt{Uniform}} 
     & GT & - & 0.00 / 0.00 & 1.00 & 0.008 & 0.00 / 0.00 & 1.00 & 0.009 \\
     \cmidrule(l){2-9}
     & MTR~\cite{shi2022motion}  & - & 0.73 / 1.58 & 0.30 & 0.062 & 0.73 / 1.59 & 0.31 & 0.061 \\
     & A-VRNN~\cite{monti2020dagnet}  & - & 1.80 / 4.63 & 0.06 & 0.057 & 1.82 / 4.67  & 0.06  & 0.058  \\
\midrule[0.7pt]

\multirow{4}{*}{\texttt{Clusters}~\cite{ye2023improving}} 
     & GT & - & 0.00 / 0.00 & 1.00 & 0.009 & 0.00 / 0.00 & 1.00 & 0.007 \\
     \cmidrule(l){2-9}
     & MTR~\cite{shi2022motion} & - & 0.69 / 1.50 & 0.35 & 0.060 & 0.71 / 1.55 & 0.33 & 0.051 \\
     & A-VRNN~\cite{monti2020dagnet}  & - & 1.79 / 4.59 & 0.08 & 0.062 & 1.82 / 4.70  & 0.07  & 0.049 \\
\midrule[0.7pt]

\multirow{10}{*}{\texttt{Scoring}} 
     & GT & - & 0.00 / 0.00 & 1.00 & 0.005 & 0.00 / 0.00 & 1.00 & 0.017 \\
 \cmidrule(l){2-9}
& \multirow{3}{*}
    {MTR~\cite{shi2022motion}}  & - &    0.72 / 1.59 & 0.32 & 0.044 & 0.74 / 1.59  & 0.30  & 0.100  \\
     & & F+~\cite{ye2023improving} &       0.73 / 1.59 & 0.32 & 0.043 & 0.75 / 1.59  & 0.30  & 0.099  \\
     &  & Ours &   0.83 / 1.80 & 0.25 & 0.037 & 0.89 / 1.91  & 0.22  & 0.086  \\ 
     \cmidrule(l){2-9}
& \multirow{3}{*}
    {A-VRNN~\cite{monti2020dagnet}}  & - &    1.99 / 5.26 & 0.05 & 0.042 & 2.13 / 5.55  & 0.05 & 0.099  \\
     & & F+~\cite{ye2023improving} &             2.05 / 5.24 & 0.06 & 0.041 & 2.23 / 5.73  & 0.06  & 0.103  \\
     &  & Ours &          1.76 / 4.58 & 0.07 & 0.041 & 1.89 / 4.87 & 0.06 & 0.095  \\ 
\bottomrule
\end{tabular}
}
\begin{tablenotes}
\scriptsize
\item \textbf{GT}: Ground truth tracks, \textbf{F+}: Fren\'et+ Strategy~\cite{ye2023improving}
\end{tablenotes}
% \vspace{-0.2cm}
\end{table*}

==> tables/main_table_v4.tex <==

\begin{table*}[!ht]
\centering
\caption{Main Experiments in WOMD~\cite{ettinger2021large}: values for ADE / FDE are in meters, collisions are rates per predicted trajectory \task{Consider changing Scoring to Proposed, and make it easier to get the main point from. What percentage increase/decrease should we include? Ideally can show increase from Validation set for collision, and increase from GT test}} \label{tab:results_main}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{c@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}}
\begin{tabular}{clccccccc}
\toprule
\multirow{2}{*}{\textbf{Data Split}} & \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Remediation}} & \multicolumn{3}{c}{\textbf{Validation Set (In-Distribution)}} & \multicolumn{3}{c}{\textbf{Testing Set (Out-of-Distribution)}}  \\ 
%\cmidrule(l){4-6} \cmidrule(l){7-9}
 & & & ADE / FDE ($\downarrow$) & mAP ($\uparrow$) & Collisions ($\downarrow$) & ADE / FDE ($\downarrow$) & mAP ($\uparrow$) & Collisions ($\downarrow$) \\ 
\midrule
\multirow{4}{*}{\texttt{Uniform}} 
     & GT & - & 0.00 / 0.00 & 1.00 & 0.008 & 0.00 / 0.00 & 1.00 & 0.009 \\
     \cmidrule(l){2-9}
%\multirow{2}{*}{\texttt{Uniform}} 
     & MTR~\cite{shi2022motion}  & - & 0.73 / 1.58 & 0.30 & 0.062 & 0.73 / 1.59 & 0.31 & 0.061 \\
     & A-VRNN~\cite{monti2020dagnet}  & - & 1.80 / 4.63 & 0.06 & 0.057 & 1.82 / 4.67  & 0.06  & 0.058  \\
\midrule[0.7pt]

\multirow{4}{*}{\texttt{Clusters}~\cite{ye2023improving}} 
     & GT & - & 0.00 / 0.00 & 1.00 & 0.009 & 0.00 / 0.00 & 1.00 & 0.007 \\
     \cmidrule(l){2-9}
%\multirow{2}{*}{\texttt{Clusters}~\cite{ye2023improving}} 
     & MTR~\cite{shi2022motion} & - & 0.69 / 1.50 & 0.35 & 0.060 & 0.71 / 1.55 & 0.33 & 0.051 \\
     & A-VRNN~\cite{monti2020dagnet}  & - & 1.79 / 4.59 & 0.08 & 0.062 & 1.82 / 4.70  & 0.07  & 0.049 \\
\midrule[0.7pt]

%\multirow{6}{*}{\texttt{Clusters}~\cite{ye2023improving}} 
%& \multirow{3}{*}
    %{MTR~\cite{shi2022motion}}  & - & 0.69 / 1.50 & 0.35 & 0.060 & 0.71 / 1.55 & 0.33 & 0.051  \\
     %& & F+~\cite{ye2023improving} &       0.73 / 1.59 & 0.32 & 0.043 & 0.75 / 1.59  & 0.30  & 0.099  \\
     %&  & Ours &   0.83 / 1.80 & 0.25 & 0.037 & 0.89 / 1.91  & 0.22  & 0.086  \\ 
     %\cmidrule(l){2-9}
%& \multirow{3}{*}
    %{A-VRNN~\cite{monti2020dagnet}}  & - & 1.79 / 4.59 & 0.08 & 0.062 & 1.82 / 4.70  & 0.07  & 0.049  \\
     %& & F+~\cite{ye2023improving} &             2.05 / 5.24 & 0.06 & 0.041 & 2.23 / 5.73  & 0.06  & 0.103  \\
     %&  & Ours &          1.76 / 4.58 & 0.07 & 0.041 & 1.89 / 4.87 & 0.06 & 0.095  \\ 
%\midrule[0.7pt]

\multirow{10}{*}{\texttt{Scoring}} 
     & GT & - & 0.00 / 0.00 & 1.00 & 0.005 & 0.00 / 0.00 & 1.00 & 0.017 \\
 \cmidrule(l){2-9}
%\multirow{6}{*}{\texttt{Scoring}} 
& \multirow{3}{*}
    {MTR~\cite{shi2022motion}}  & - &    0.72 / 1.59 & 0.32 & 0.044 & 0.74 / 1.59  & 0.30  & 0.100  \\
     & & F+~\cite{ye2023improving} &       0.73 / 1.59 & 0.32 & 0.043 & 0.75 / 1.59  & 0.30  & 0.099  \\
     &  & Ours &   0.83 / 1.80 & 0.25 & 0.037 & 0.89 / 1.91  & 0.22  & 0.086  \\ 
     \cmidrule(l){2-9}
& \multirow{3}{*}
    {A-VRNN~\cite{monti2020dagnet}}  & - &    1.99 / 5.26 & 0.05 & 0.042 & 2.13 / 5.55  & 0.05 & 0.099  \\
     & & F+~\cite{ye2023improving} &             2.05 / 5.24 & 0.06 & 0.041 & 2.23 / 5.73  & 0.06  & 0.103  \\
     %&  & Ours &          1.76 / 4.58 & 0.07 & 0.041 & 1.89 / 4.87 & 0.06 & 0.095  \\ 
     &  & Ours &          1.76 / 4.61 & 0.06 & 0.039 & 1.91 / 4.94 & 0.06 & 0.093  \\ 
\bottomrule
\end{tabular}
}
\begin{tablenotes}
\scriptsize
\item \textbf{GT}: Ground truth tracks, \textbf{F+}: Fren\'et+ Strategy~\cite{ye2023improving}
\end{tablenotes}
\vspace{-0.5cm}
\end{table*}

==> tables/main_table_v5.tex <==

\begin{table*}[!ht]
\centering
\caption{Main Experiments in WOMD~\cite{ettinger2021large}. ADE / FDE in meters, CR is collision rate per predicted trajectory. $\Delta_{val}$ and $\Delta_{test}$ are the change in test CR from the \textit{un-remediated} val and test for the given data split and method.} \label{tab:results_main}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{c@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}}
\begin{tabular}{clcccccc}
%\begin{tabular}{clcclccl}
\toprule
\multirow{2}{*}{\textbf{Data Split}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Validation Set (In-Distribution)}} & \multicolumn{3}{c}{\textbf{Testing Set (Out-of-Distribution)}}  \\ 
%\cmidrule(l){4-6} \cmidrule(l){7-9}
 & & ADE / FDE  & mAP  & CR  & ADE / FDE  & mAP  & CR ($\Delta_{val}$, $\Delta_{test}$) \\ 
\midrule
\multirow{3}{*}{\texttt{Uniform}} 
     %& GT  & - / - & - & 0.008 & - / - & - & 0.009 ($+12.5\%$, $-0.00\%$) \\
     & GT  & - / - & - & 0.008 & - / - & - & 0.009 ($+12.5\%$, -) \\
     
     %\cmidrule(l){2-8}
%\multirow{2}{*}{\texttt{Uniform}} 
     %& MTR~\cite{shi2022motion}   & 0.73 / 1.58 & 0.30 & 0.062 & 0.73 / 1.59 & 0.31 & 0.061 ($-1.60\%$, $-0.00\%$)\\
     & MTR~\cite{shi2022motion}   & 0.73 / 1.58 & 0.30 & 0.062 & 0.73 / 1.59 & 0.31 & 0.061 ($-1.60\%$, -)\\
     %\cmidrule(l){2-8}
     %& A-VRNN~\cite{monti2020dagnet}   & 1.80 / 4.63 & 0.06 & 0.057 & 1.82 / 4.67  & 0.06  & 0.058 ($+1.80\%$, $-0.00\%$) \\
     & A-VRNN~\cite{monti2020dagnet}   & 1.80 / 4.63 & 0.06 & 0.057 & 1.82 / 4.67  & 0.06  & 0.058 ($+1.80\%$, -) \\
\midrule[0.7pt]

\multirow{3}{*}{\texttt{Clusters}~\cite{ye2023improving}} 
     %& GT  & 0.00 / 0.00 & 1.00 & 0.009 & 0.00 / 0.00 & 1.00 & 0.007 ($-22.2\%$, $-0.0\%$) \\
     %& GT  & - / - & - & 0.009 & - / - & - & 0.007 ($-22.2\%$, $-0.00\%$) \\
     & GT  & - / - & - & 0.009 & - / - & - & 0.007 ($-22.2\%$, -) \\
     
     %\cmidrule(l){2-8}
%\multirow{2}{*}{\texttt{Clusters}~\cite{ye2023improving}} 
     %& MTR~\cite{shi2022motion} & 0.69 / 1.50 & 0.35 & 0.060 & 0.71 / 1.55 & 0.33 & 0.051 ($-15.0\%$,  $-0.00\%$)\\
     & MTR~\cite{shi2022motion} & 0.69 / 1.50 & 0.35 & 0.060 & 0.71 / 1.55 & 0.33 & 0.051 ($-15.0\%$,  -)\\
     %\cmidrule(l){2-8}
     %& A-VRNN~\cite{monti2020dagnet}   & 1.79 / 4.59 & 0.08 & 0.062 & 1.82 / 4.70  & 0.07  & 0.049 ($-21.0\%$, $-0.00\%$)\\
     & A-VRNN~\cite{monti2020dagnet}   & 1.79 / 4.59 & 0.08 & 0.062 & 1.82 / 4.70  & 0.07  & 0.049 ($-21.0\%$, -)\\
\midrule[0.7pt]

%\multirow{6}{*}{\texttt{Clusters}~\cite{ye2023improving}} 
%& \multirow{3}{*}
    %{MTR~\cite{shi2022motion}}  & - & 0.69 / 1.50 & 0.35 & 0.060 & 0.71 / 1.55 & 0.33 & 0.051  \\
     %& & F+~\cite{ye2023improving} &       0.73 / 1.59 & 0.32 & 0.043 & 0.75 / 1.59  & 0.30  & 0.099  \\
     %&  & Ours &   0.83 / 1.80 & 0.25 & 0.037 & 0.89 / 1.91  & 0.22  & 0.086  \\ 
     %\cmidrule(l){2-9}
%& \multirow{3}{*}
    %{A-VRNN~\cite{monti2020dagnet}}  & - & 1.79 / 4.59 & 0.08 & 0.062 & 1.82 / 4.70  & 0.07  & 0.049  \\
     %& & F+~\cite{ye2023improving} &             2.05 / 5.24 & 0.06 & 0.041 & 2.23 / 5.73  & 0.06  & 0.103  \\
     %&  & Ours &          1.76 / 4.58 & 0.07 & 0.041 & 1.89 / 4.87 & 0.06 & 0.095  \\ 
%\midrule[0.7pt]

\multirow{7}{*}{\texttt{Scoring} (Ours)} 
     %& GT  & 0.00 / 0.00 & 1.00 & 0.005 & 0.00 / 0.00 & 1.00 & 0.017 ($+240\%$, $+0.0\%$) \\
     & GT  & - / - & - & 0.005 & - / - & - & 0.017 ($+240\%$, -) \\
 \cmidrule(l){2-8}
%\multirow{6}{*}{\texttt{Scoring}} 
%& MTR~\cite{shi2022motion}   &    0.72 / 1.59 & 0.32 & 0.044 & 0.74 / 1.59  & 0.30  & 0.100 ($+127\%$, $-0.00\%$) \\
& MTR~\cite{shi2022motion}   &    0.72 / 1.59 & 0.32 & 0.044 & 0.74 / 1.59  & 0.30  & 0.100 ($+127\%$, -) \\
     & MTR~\cite{shi2022motion} + F+~\cite{ye2023improving} &       0.73 / 1.59 & 0.32 & 0.043 & 0.75 / 1.59  & 0.30  & 0.099 ($+125\%$, $-1.00\%$)  \\
     & MTR~\cite{shi2022motion} + Ours &   0.83 / 1.80 & 0.25 & 0.037 & 0.89 / 1.91  & 0.22  & 0.086 ($+95.5\%$, $-14.0\%$) \\ 
     \cmidrule(l){2-8}
%& A-VRNN~\cite{monti2020dagnet}   &    1.99 / 5.26 & 0.05 & 0.042 & 2.13 / 5.55  & 0.05 & 0.099 ($+136\%$, $-0.00\%$) \\
& A-VRNN~\cite{monti2020dagnet}   &    1.99 / 5.26 & 0.05 & 0.042 & 2.13 / 5.55  & 0.05 & 0.099 ($+136\%$, -) \\
     & A-VRNN~\cite{monti2020dagnet} + F+~\cite{ye2023improving} &             2.05 / 5.24 & 0.06 & 0.041 & 2.23 / 5.73  & 0.06  & 0.103 ($+145\%$, $+4.04\%$ \\
     %&  & Ours &          1.76 / 4.58 & 0.07 & 0.041 & 1.89 / 4.87 & 0.06 & 0.095  \\ 
     &  A-VRNN~\cite{monti2020dagnet} + Ours &          1.76 / 4.61 & 0.06 & 0.039 & 1.91 / 4.94 & 0.06 & 0.093 ($+121\%$, $-6.06\%$) \\ 
\bottomrule
\end{tabular}
}
\begin{tablenotes}
\scriptsize
\item \textbf{GT}: Ground truth tracks, \textbf{F+}: Fren\'et+ Strategy~\cite{ye2023improving}
\end{tablenotes}
\vspace{-0.5cm}
\end{table*}

==> tables/main_table_v6.tex <==

\begin{table*}[!ht]
\vspace{0.4cm}
\centering
\caption{Distribution shift experiments in WOMD~\cite{ettinger2021large}. ADE / FDE is in meters. $\Delta_{val}$ and $\Delta_{test}$ are the change in test CR from the \textit{un-remediated} val and test for the given data split and method. The best remediation result is \textbf{bolded}.} \label{tab:results_main}
%\resizebox{0.95\textwidth}{!}{%
\resizebox{\textwidth}{!}{%
% \begin{tabular}{c@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}}
\begin{tabular}{clcccccl}
%\begin{tabular}{clcclccl}
\toprule
\multirow{2}{*}{\textbf{Data Split}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Validation Set (In-Distribution)}} & \multicolumn{3}{c}{\textbf{Testing Set (Out-of-Distribution)}}  \\ 
%\cmidrule(l){4-6} \cmidrule(l){7-9}
 & & ADE / FDE  & mAP  & CR  & ADE / FDE  & mAP  & \ \ CR \ ($\Delta_{val}$, \ \ \ \ \ \ \ $\Delta_{test}$\ \ ) \\ 
\midrule
\multirow{3}{*}{\texttt{Uniform}} 
     %& GT  & - / - & - & 0.008 & - / - & - & 0.009 ($+12.5\%$, $-0.00\%$) \\
     & GT  & - / - & - & 0.008 & - / - & - & 0.009 ($+12.5\%$, \qquad \ - \quad \ ) \\
     
     %\cmidrule(l){2-8}
%\multirow{2}{*}{\texttt{Uniform}} 
     %& MTR~\cite{shi2022motion}   & 0.73 / 1.58 & 0.30 & 0.062 & 0.73 / 1.59 & 0.31 & 0.061 ($-1.60\%$, $-0.00\%$)\\
     & MTR~\cite{shi2022motion}   & 0.73 / 1.58 & 0.30 & 0.062 & 0.73 / 1.59 & 0.31 & 0.061 ($-1.60\%$, \qquad \ - \quad \ )\\
     %\cmidrule(l){2-8}
     %& A-VRNN   & 1.80 / 4.63 & 0.06 & 0.057 & 1.82 / 4.67  & 0.06  & 0.058 ($+1.80\%$, $-0.00\%$) \\
     & A-VRNN~\cite{monti2020dagnet}   & 1.80 / 4.63 & 0.06 & 0.057 & 1.82 / 4.67  & 0.06  & 0.058 ($+1.80\%$, \qquad \ - \quad \ ) \\
\midrule[0.7pt]

\multirow{3}{*}{\texttt{Clusters}~\cite{ye2023improving}} 
     %& GT  & 0.00 / 0.00 & 1.00 & 0.009 & 0.00 / 0.00 & 1.00 & 0.007 ($-22.2\%$, $-0.0\%$) \\
     %& GT  & - / - & - & 0.009 & - / - & - & 0.007 ($-22.2\%$, $-0.00\%$) \\
     & GT  & - / - & - & 0.009 & - / - & - & 0.007 ($-22.2\%$, \qquad \ - \quad \ ) \\
     
     %\cmidrule(l){2-8}
%\multirow{2}{*}{\texttt{Clusters}~\cite{ye2023improving}} 
     %& MTR~\cite{shi2022motion} & 0.69 / 1.50 & 0.35 & 0.060 & 0.71 / 1.55 & 0.33 & 0.051 ($-15.0\%$,  $-0.00\%$)\\
     & MTR & 0.69 / 1.50 & 0.35 & 0.060 & 0.71 / 1.55 & 0.33 & 0.051 ($-15.0\%$,  \qquad \ - \quad \ )\\
     %\cmidrule(l){2-8}
     %& A-VRNN   & 1.79 / 4.59 & 0.08 & 0.062 & 1.82 / 4.70  & 0.07  & 0.049 ($-21.0\%$, $-0.00\%$)\\
     & A-VRNN   & 1.79 / 4.59 & 0.08 & 0.062 & 1.82 / 4.70  & 0.07  & 0.049 ($-21.0\%$, \qquad \ - \quad \ )\\
\midrule[0.7pt]

%\multirow{6}{*}{\texttt{Clusters}~\cite{ye2023improving}} 
%& \multirow{3}{*}
    %{MTR~\cite{shi2022motion}}  & - & 0.69 / 1.50 & 0.35 & 0.060 & 0.71 / 1.55 & 0.33 & 0.051  \\
     %& & F+~\cite{ye2023improving} &       0.73 / 1.59 & 0.32 & 0.043 & 0.75 / 1.59  & 0.30  & 0.099  \\
     %&  & Ours &   0.83 / 1.80 & 0.25 & 0.037 & 0.89 / 1.91  & 0.22  & 0.086  \\ 
     %\cmidrule(l){2-9}
%& \multirow{3}{*}
    %{A-VRNN}  & - & 1.79 / 4.59 & 0.08 & 0.062 & 1.82 / 4.70  & 0.07  & 0.049  \\
     %& & F+~\cite{ye2023improving} &             2.05 / 5.24 & 0.06 & 0.041 & 2.23 / 5.73  & 0.06  & 0.103  \\
     %&  & Ours &          1.76 / 4.58 & 0.07 & 0.041 & 1.89 / 4.87 & 0.06 & 0.095  \\ 
%\midrule[0.7pt]

\multirow{7}{*}{\texttt{Scoring} (Ours)} 
     %& GT  & 0.00 / 0.00 & 1.00 & 0.005 & 0.00 / 0.00 & 1.00 & 0.017 ($+240\%$, $+0.0\%$) \\
     & GT  & - / - & - & 0.005 & - / - & - & 0.017 ($+240\%$, \qquad \ - \ \quad \ ) \\
 \cmidrule(l){2-8}
%\multirow{6}{*}{\texttt{Scoring}} 
%& MTR~\cite{shi2022motion}   &    0.72 / 1.59 & 0.32 & 0.044 & 0.74 / 1.59  & 0.30  & 0.100 ($+127\%$, $-0.00\%$) \\
& MTR   &    0.72 / 1.59 & 0.32 & 0.044 & 0.74 / 1.59  & 0.30  & 0.100 ($+127\%$, \qquad \ \ - \quad \ ) \\
     & MTR + F+~\cite{ye2023improving} &       0.73 / 1.59 & 0.32 & 0.043 & 0.75 / 1.59  & 0.30  & 0.099 ($+125\%$, \ \  $-1.00\%$ )  \\
     & MTR + Ours &   0.83 / 1.80 & 0.25 & 0.037 & 0.89 / 1.91  & 0.22  & \textbf{0.086} ($\mathbf{+95.5\%}$, $\mathbf{-14.0\%}$ ) \\ 
     \cmidrule(l){2-8}
%& A-VRNN   &    1.99 / 5.26 & 0.05 & 0.042 & 2.13 / 5.55  & 0.05 & 0.099 ($+136\%$, $-0.00\%$) \\
& A-VRNN   &    1.99 / 5.26 & 0.05 & 0.042 & 2.13 / 5.55  & 0.05 & 0.099 ($+136\%$, \qquad \ \ - \quad \ ) \\
     & A-VRNN + F+ &             2.05 / 5.24 & 0.06 & 0.041 & 2.23 / 5.73  & 0.06  & 0.103 ($+145\%$, \ \ $+4.04\%$ ) \\
     %&  & Ours &          1.76 / 4.58 & 0.07 & 0.041 & 1.89 / 4.87 & 0.06 & 0.095  \\ 
     &  A-VRNN + Ours &          1.76 / 4.61 & 0.06 & 0.039 & 1.91 / 4.94 & 0.06 & \textbf{0.093} ($\mathbf{+121\%}$, \  $\mathbf{-6.06\%}$ ) \\ 
\bottomrule
\end{tabular}
}
\begin{tablenotes}
\scriptsize
\item \textbf{GT}: Ground truth tracks, \textbf{F+}: Fren\'et+ Strategy~\cite{ye2023improving}
\end{tablenotes}
\vspace{-0.5cm}
\end{table*}

==> tables/main_table_v7.tex <==

\begin{table*}[!ht]
\vspace{0.2cm}
\centering
\caption{Main Experiments in WOMD~\cite{ettinger2021large}. ADE / FDE in meters, CR is collision rate per predicted trajectory. $\Delta_{val}$ and $\Delta_{test}$ are the change in test CR from the \textit{un-remediated} val and \textit{ground truth} test for the given data split and method. The best remediation result is \textbf{bolded}.} \label{tab:results_main}
\resizebox{\textwidth}{!}{%
% \begin{tabular}{c@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}}
\begin{tabular}{clcccccl}
%\begin{tabular}{clcclccl}
\toprule
\multirow{2}{*}{\textbf{Data Split}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Validation Set (In-Distribution)}} & \multicolumn{3}{c}{\textbf{Testing Set (Out-of-Distribution)}}  \\ 
%\cmidrule(l){4-6} \cmidrule(l){7-9}
 & & ADE / FDE  & mAP  & CR  & ADE / FDE  & mAP  & \ \ CR \ ($\Delta_{val}$, \ \ \ \ \ \ \ $\Delta_{test}$\ \ ) \\ 
\midrule
\multirow{3}{*}{\texttt{Uniform}} 
     %& GT  & - / - & - & 0.008 & - / - & - & 0.009 ($+12.5\%$, $-0.00\%$) \\
     & GT  & - / - & - & 0.008 & - / - & - & 0.009 ($+12.5\%$, \qquad \ - \quad \ ) \\
     
     %\cmidrule(l){2-8}
%\multirow{2}{*}{\texttt{Uniform}} 
     %& MTR~\cite{shi2022motion}   & 0.73 / 1.58 & 0.30 & 0.062 & 0.73 / 1.59 & 0.31 & 0.061 ($-1.60\%$, $-0.00\%$)\\
     & MTR~\cite{shi2022motion}   & 0.73 / 1.58 & 0.30 & 0.062 & 0.73 / 1.59 & 0.31 & 0.061 ($-1.60\%$, \ $+578\%$ \ )\\
     %\cmidrule(l){2-8}
     %& A-VRNN~\cite{monti2020dagnet}   & 1.80 / 4.63 & 0.06 & 0.057 & 1.82 / 4.67  & 0.06  & 0.058 ($+1.80\%$, $-0.00\%$) \\
     & A-VRNN~\cite{monti2020dagnet}   & 1.80 / 4.63 & 0.06 & 0.057 & 1.82 / 4.67  & 0.06  & 0.058 ($+1.80\%$, \ $+544\%$ \  ) \\
\midrule[0.7pt]

\multirow{3}{*}{\texttt{Clusters}~\cite{ye2023improving}} 
     %& GT  & 0.00 / 0.00 & 1.00 & 0.009 & 0.00 / 0.00 & 1.00 & 0.007 ($-22.2\%$, $-0.0\%$) \\
     %& GT  & - / - & - & 0.009 & - / - & - & 0.007 ($-22.2\%$, $-0.00\%$) \\
     & GT  & - / - & - & 0.009 & - / - & - & 0.007 ($-22.2\%$, \qquad \ - \quad \ ) \\
     
     %\cmidrule(l){2-8}
%\multirow{2}{*}{\texttt{Clusters}~\cite{ye2023improving}} 
     %& MTR~\cite{shi2022motion} & 0.69 / 1.50 & 0.35 & 0.060 & 0.71 / 1.55 & 0.33 & 0.051 ($-15.0\%$,  $-0.00\%$)\\
     & MTR~\cite{shi2022motion} & 0.69 / 1.50 & 0.35 & 0.060 & 0.71 / 1.55 & 0.33 & 0.051 ($-15.0\%$,  \ $+629\%$ \ )\\
     %\cmidrule(l){2-8}
     %& A-VRNN~\cite{monti2020dagnet}   & 1.79 / 4.59 & 0.08 & 0.062 & 1.82 / 4.70  & 0.07  & 0.049 ($-21.0\%$, $-0.00\%$)\\
     & A-VRNN~\cite{monti2020dagnet}   & 1.79 / 4.59 & 0.08 & 0.062 & 1.82 / 4.70  & 0.07  & 0.049 ($-21.0\%$, \ $+600\%$ \ )\\
\midrule[0.7pt]

%\multirow{6}{*}{\texttt{Clusters}~\cite{ye2023improving}} 
%& \multirow{3}{*}
    %{MTR~\cite{shi2022motion}}  & - & 0.69 / 1.50 & 0.35 & 0.060 & 0.71 / 1.55 & 0.33 & 0.051  \\
     %& & F+~\cite{ye2023improving} &       0.73 / 1.59 & 0.32 & 0.043 & 0.75 / 1.59  & 0.30  & 0.099  \\
     %&  & Ours &   0.83 / 1.80 & 0.25 & 0.037 & 0.89 / 1.91  & 0.22  & 0.086  \\ 
     %\cmidrule(l){2-9}
%& \multirow{3}{*}
    %{A-VRNN~\cite{monti2020dagnet}}  & - & 1.79 / 4.59 & 0.08 & 0.062 & 1.82 / 4.70  & 0.07  & 0.049  \\
     %& & F+~\cite{ye2023improving} &             2.05 / 5.24 & 0.06 & 0.041 & 2.23 / 5.73  & 0.06  & 0.103  \\
     %&  & Ours &          1.76 / 4.58 & 0.07 & 0.041 & 1.89 / 4.87 & 0.06 & 0.095  \\ 
%\midrule[0.7pt]

\multirow{7}{*}{\texttt{Scoring} (Ours)} 
     %& GT  & 0.00 / 0.00 & 1.00 & 0.005 & 0.00 / 0.00 & 1.00 & 0.017 ($+240\%$, $+0.0\%$) \\
     & GT  & - / - & - & 0.005 & - / - & - & 0.017 ($+240\%$, \qquad \ - \ \quad \ ) \\
 \cmidrule(l){2-8}
%\multirow{6}{*}{\texttt{Scoring}} 
%& MTR~\cite{shi2022motion}   &    0.72 / 1.59 & 0.32 & 0.044 & 0.74 / 1.59  & 0.30  & 0.100 ($+127\%$, $-0.00\%$) \\
& MTR~\cite{shi2022motion}   &    0.72 / 1.59 & 0.32 & 0.044 & 0.74 / 1.59  & 0.30  & 0.100 ($+127\%$, \ $+488\%$ \ \ ) \\
     & MTR~\cite{shi2022motion} + F+~\cite{ye2023improving} &       0.73 / 1.59 & 0.32 & 0.043 & 0.75 / 1.59  & 0.30  & 0.099 ($+125\%$,  \ $+482\%$ \ \ )  \\
     & MTR~\cite{shi2022motion} + Ours &   0.83 / 1.80 & 0.25 & 0.037 & 0.89 / 1.91  & 0.22  & \textbf{0.086} ($\mathbf{+95.5\%}$, $\mathbf{+406\%}$ \  ) \\ 
     \cmidrule(l){2-8}
%& A-VRNN~\cite{monti2020dagnet}   &    1.99 / 5.26 & 0.05 & 0.042 & 2.13 / 5.55  & 0.05 & 0.099 ($+136\%$, $-0.00\%$) \\
& A-VRNN~\cite{monti2020dagnet}   &    1.99 / 5.26 & 0.05 & 0.042 & 2.13 / 5.55  & 0.05 & 0.099 ($+136\%$, \ $+482\%$ \ \ ) \\
     & A-VRNN~\cite{monti2020dagnet} + F+~\cite{ye2023improving} &             2.05 / 5.24 & 0.06 & 0.041 & 2.23 / 5.73  & 0.06  & 0.103 ($+145\%$, \ $+506\%$ \ \ ) \\
     %&  & Ours &          1.76 / 4.58 & 0.07 & 0.041 & 1.89 / 4.87 & 0.06 & 0.095  \\ 
     &  A-VRNN~\cite{monti2020dagnet} + Ours &          1.76 / 4.61 & 0.06 & 0.039 & 1.91 / 4.94 & 0.06 & \textbf{0.093} ($\mathbf{+121\%}$, \ $\mathbf{+447\%}$ \ ) \\ 
\bottomrule
\end{tabular}
}
\begin{tablenotes}
\scriptsize
\item \textbf{GT}: Ground truth tracks, \textbf{F+}: Fren\'et+ Strategy~\cite{ye2023improving}
\end{tablenotes}
\vspace{-0.5cm}
\end{table*}

==> tables/remediation_ablation_old.tex <==
\begin{table*}[!ht]
\vspace{0.4cm}
\centering
\caption{Remediation strategy ablation study based on our proposed approach in \Cref{ssec:remediation_approach}. Results are on WOMD~\cite{ettinger2021large}. } \label{tab:results_remediation}
%\resizebox{0.95\textwidth}{!}{%
\resizebox{\textwidth}{!}{%
% \begin{tabular}{c@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}ccc@{\hspace{0.3cm}}}
\begin{tabular}{lcccccccc@{}}
\toprule

\multirow{2}{*}{\textbf{Method Name}} & \multicolumn{2}{c}{\textbf{Scoring Strategy}} & \multicolumn{3}{c}{\textbf{Validation Set (In-Distribution)}} & \multicolumn{3}{c}{\textbf{Testing Set (Out-of-Distribution)}}  \\ 

%\cmidrule(l){2-3} \cmidrule(l){4-6} \cmidrule(l){7-9}
  %& SC & CL & ADE / FDE ($\downarrow$) & mAP ($\uparrow$) & Collisions ($\downarrow$) & ADE / FDE ($\downarrow$) & mAP ($\uparrow$) & Collisions ($\downarrow$) \\
  & SC & CL & ADE / FDE & mAP  & CR & ADE / FDE  & mAP & CR ($\Delta_{val}$, \ \ \ \ \ \ \ $\Delta_{test}$\ ) \\
  \midrule
   MTR~\cite{shi2022motion} & - & - & 0.72 / 1.59 & 0.32 & 0.044 & 0.74 / 1.59  & 0.30  & 0.100 ($+127\%$, \ \ \ \ \ \ - \ \ \ \ ) \\
   MTR + Ours (SC only)  & $\checkmark$ & - & 0.74 / 1.63 & 0.31 & 0.046 & 0.74 / 1.61 & 0.29 & 0.103 ($+134\%$, \ $+3.00\%$\ ) \\
   MTR + Ours (CL only) & - & $\checkmark$ & 0.81 / 1.77 & 0.27 & 0.038 & 0.88 / 1.92 & 0.23 & 0.093 ($+111\%$, \ $-7.00\%$\ ) \\
   MTR + Ours (Full) & $\checkmark$ & $\checkmark$ & 0.83 / 1.80 & 0.25 & 0.037 & 0.89 / 1.91  & 0.22  & \textbf{0.086 ($+\textbf{95.5}\%$, \   $-\textbf{14.0}\%$\ )} \\
\bottomrule
\end{tabular}
}
\begin{tablenotes}
\scriptsize
\item \textbf{SC}: Score incorporation, \textbf{CL}: Collision loss objective.
\end{tablenotes}
\vspace{-0.5cm}
\end{table*}

==> tables/score_ablation_gt.tex <==

\begin{table*}[!ht]
\centering
\caption{Scoring strategy ablation. Using GT and FE combined, with asymmetric scoring, results in the highest absolute and relative increase in collision rate from ID to OOD, across three tested collision thresholds.} \label{tab:results_scoring}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lccccc@{\hskip 0.1cm}ccc@{\hskip 0.1cm}ccc@{}}
\toprule
\multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{Scoring Strategy}} & & \multicolumn{3}{c}{\textbf{Validation Set (In-Distribution)}} & & \multicolumn{3}{c}{\textbf{Testing Set (Out-of-Distribution)}}  \\ 
%\cmidrule(l){2-4} \cmidrule(l){6-8} \cmidrule(l){10-12}
& GT & FE & AS && Colls@0.25 ($\downarrow$) & Colls@0.50 ($\downarrow$) & Colls@1.0 ($\downarrow$) & & Colls@0.25 ($\downarrow$) & Colls@0.50 ($\downarrow$) & Colls@1.0 ($\downarrow$) \\ 
\midrule
\multirow{5}{*}{Ground Truth} 
    & $\checkmark$ & - & - && 0.004 & 0.042 & 0.110 && 0.015 & 0.127 & 0.308  \\
    & - & $\checkmark$ &  - && 0.006 & 0.043 & 0.121 && 0.015 & 0.124 & 0.300 \\
    & $\checkmark$ & $\checkmark$ & - && 0.007 & 0.047 & 0.125 && 0.016 & 0.126 & 0.303 \\
    & - & $\checkmark$ & $\checkmark$ && 0.004 & 0.041 & 0.115 && 0.016 & 0.129 & 0.309 \\
    & $\checkmark$ & $\checkmark$ & $\checkmark$ && 0.005 & 0.044 & 0.118 && 0.017 & 0.131 & 0.311 \\
\bottomrule
\end{tabular}
}
\begin{tablenotes}
\scriptsize
\item \textbf{GT}: Ground truth, \textbf{FE}: Future extrapolated, \textbf{AS}: Asymmetric.
\end{tablenotes}
\vspace{-0.2cm}
\end{table*}

==> tables/stats_table.tex <==
\begin{table}[!ht]
\centering
\caption{Dataset Split Statistics \task{Determine what else to put here, if anything? Perhaps GT collision rate, mean/std of various metrics, etc.}} \label{tab:dataset_stats}
\resizebox{0.48\textwidth}{!}{%
%\begin{tabular}{@{}lcccccc}
\begin{tabular}{@{}lccc}
\toprule
\multirow{2}{*}{\textbf{Metric}} & \multicolumn{3}{c}{\textbf{Splitting Scheme}}  \\ 
%\textbf{Split} & Train Scenes & Train Trajs & Val Scenes & Val Trajs & Test Scenes & Test Trajs \\
& \texttt{Uniform} & \texttt{Clusters} & \texttt{Scoring} \\ 
\midrule

Training Scenes & 90,289 & 105,407 & 108,759 \\
Training Trajs & 403,386 & 476,780 & 436,545 \\
\midrule
Validation Scenes & 39,818 & 26,299 & 27,193 \\
Validation Trajs & 178,127 & 118,660 & 109,192 \\
\midrule
Testing Scenes & 39,833 & 38,234 & 33,988 \\
Testing Trajs & 177,278 & 163,351 & 213,054 \\

%\texttt{Uniform} & 90,289 & 403,386 & 39,818 & 178,127 & 39,833 & 177,278 \\
%\texttt{Clusters} & 105,407 & 476,780 & 26,299 & 118,660 & 38,234 & 163,351 \\
%\texttt{Scoring} & 108,759 & 436,545 & 27,193 & 109,192 & 33,988 & 213,054 \\
\bottomrule
\end{tabular}
}
%\begin{tablenotes}
%\scriptsize
%\item \textbf{GT}: Ground truth, \textbf{FE}: Future extrapolated, \textbf{AS}: Asymmetric.
%\end{tablenotes}
\vspace{-0.2cm}
\end{table}
